Design and Evaluation of a Generic Visual SLAM Framework for Multi-Camera Systems

Multi-camera systems have been shown to improve the accuracy and robustness of SLAM estimates, yet state-of-the-art SLAM systems predominantly support monocular or stereo setups. This paper presents a generic sparse visual SLAM framework capable of running on any number of cameras and in any arrangement. Our SLAM system uses the generalized camera model, which allows us to represent an arbitrary multi-camera system as a single imaging device. Additionally, it takes advantage of the overlapping fields of view (FoV) by extracting cross-matched features across cameras in the rig. This limits the linear rise in the number of features with the number of cameras and keeps the computational load in check while enabling an accurate representation of the scene. We evaluate our method in terms of accuracy, robustness, and run time on indoor and outdoor datasets that include challenging real-world scenarios such as narrow corridors, featureless spaces, and dynamic objects. We show that our system can adapt to different camera configurations and allows real-time execution for typical robotic applications. Finally, we benchmark the impact of the critical design parameters - the number of cameras and the overlap between their FoV that define the camera configuration for SLAM. All our software and datasets are freely available for further research.

==> extra/accuracy_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t!]
%\captionsetup{font={small,it}, labelfont={bf,sf}}
\captionsetup{font=footnotesize,labelfont={bf,sf}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|ll|ll|ll|ll|ll|}
\hline
 &
  \multicolumn{2}{l|}{\textbf{ISEC Lab1}} &
  \multicolumn{2}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}ISEC Ground1\\ (non dynamic)\end{tabular}}} &
  \multicolumn{2}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}ISEC Ground2\\       (night)\end{tabular}}} &
  \multicolumn{2}{l|}{\textbf{Curry Center}} &
  \multicolumn{2}{l|}{\textbf{Falmouth}} \\ \hline
\textbf{Algorithm} &
  \multicolumn{1}{l|}{\textbf{ATE(m)}} &
  \textbf{ATE(\%)} &
  \multicolumn{1}{l|}{\textbf{ATE(m)}} &
  \textbf{ATE(\%)} &
  \multicolumn{1}{l|}{\textbf{ATE(m)}} &
  \textbf{ATE(\%)} &
  \multicolumn{1}{l|}{\textbf{ATE(m)}} &
  \textbf{ATE(\%)} &
  \multicolumn{1}{l|}{\textbf{ATE(m)}} &
  \textbf{ATE(\%)} \\ \hline
\rowcolor[HTML]{9BD3AA} 
OV 2 cams &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}2.65} &
  1.74 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.99} &
  1.07 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}2.41} &
  2.51 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}1.18} &
  1.5 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}210.02} &
  8.05 \\
\rowcolor[HTML]{9BD3AA} 
OV 3 cams &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}1.23} &
  0.81 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.350} &
  0.38 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}2.38} &
  2.47 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.482} &
  0.63 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}48.744} &
  1.87 \\
\rowcolor[HTML]{9BD3AA} 
OV 4 cams &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.84} &
  0.56 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.321} &
  0.34 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}1.61} &
  1.67 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.359} &
  0.46 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}42.179} &
  1.62 \\
\rowcolor[HTML]{9BD3AA} 
OV 5 cams &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.62} &
  0.41 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.296} &
  0.32 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}1.2} &
  1.25 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}0.292} &
  0.38 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9BD3AA}28.481} &
  1.09 \\
\rowcolor[HTML]{FFCCC9} 
\begin{tabular}[c]{@{}l@{}}N-OV 3cams\end{tabular} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}14.83} &
  9.75 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}2.01} &
  2.09 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}} &
  \cellcolor[HTML]{C0C0C0} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}1.423} &
  1.85 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} }} &
  \cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} } \\\hline
  \multicolumn{11}{|c|}{\textbf{SOTA Comparison in stereo mode}} \\ \hline
\rowcolor[HTML]{B0DCED} 
ORB SLAM3 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}2.9} &
  1.91 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}0.85} &
  0.8 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}2.98} &
  3.1 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}4.84} &
  6.3 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}49.708} &
  1.91\\
  \rowcolor[HTML]{B0DCED}
  SVO Pro &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}2.435} &
  1.6 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}0.901} &
  1.01 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}2.698} &
  2.99 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}41.236} &
  11.87 &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B0DCED}61.38} &
  2.19\\ \hline
 \end{tabular}%
}
\caption{Absolute translation error(ATE) of the proposed method and two state of the art SLAM systems SVO(stereo) and ORBSLAM3(stereo) with respect to the ground truth for different sequences. Our method uses both overlapping (OV) and non-overlapping (N-OV) configurations. The OV configuration results are shown in green where we choose cameras from the front-facing array starting with the stereo setup (used for ORBSLAM3 and SVO) and, adding one camera for each run. For the N-OV configuration shown in pink we choose the three cameras enclosed in blue box shown in \cref{fig:camera_rig}. Note that for the ISEC\_Ground2 and Falmouth sequences we do not have non-overlapping data. The table shows that the stereo configurations for all systems are roughly comparable but there are significant gains in using an increasing number of cameras.}
\label{tab:slam_accuracy}
\vspace{-4mm}
\end{table*}

==> extra/mcslam_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\captionsetup{font=footnotesize,labelfont={bf,sf}}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|ll|ll|ll|}
\hline
\multirow{2}{*}{} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Trajectory\\ length (m)\end{tabular}}} &
  \multicolumn{2}{l|}{\textbf{MCSLAM}} &
  \multicolumn{2}{l|}{\textbf{MultiColSLAM}} &
  \multicolumn{2}{l|}{\textbf{MCPTAM}} \\ \cline{3-8} 
 &
   &
  \multicolumn{1}{l|}{\textbf{OV}} &
  \textbf{N-OV} &
  \multicolumn{1}{l|}{\textbf{OV}} &
  \textbf{N-OV} &
  \multicolumn{1}{l|}{\textbf{OV}} &
  \textbf{N-OV} \\ \hline
\textbf{Plus} &
  11.754 &
  \multicolumn{1}{l|}{0.021} &
  0.128 &
  \multicolumn{1}{l|}{0.188} &
  0.23 &
  \multicolumn{1}{l|}{} &
   \\
\textbf{Square} &
  9.898 &
  \multicolumn{1}{l|}{0.012} &
  0.121 &
  \multicolumn{1}{l|}{0.114} &
  0.74 &
  \multicolumn{1}{l|}{} &
   \\
\textbf{Circle} &
  11.166 &
  \multicolumn{1}{l|}{0.054} &
  0.58 &
  \multicolumn{1}{l|}{0.03} &
  0.031 &
  \multicolumn{1}{l|}{} &
   \\ \hline
\end{tabular}%
}
\caption{This shows a comparison of the trajectory errors with respect to MultiColSLAM, which is our baseline multi-camera SLAM method in both overlapping and non-overlapping setups on some simple sequences with optitrack groundtruth.}
\label{tab:mcslam_compare}
\vspace{-2mm}
\end{table}

%\caption{This shows a comparison of the trajectory errors with respect to the baseline multi-camera SLAM methods in overlapping and non-overlapping setups.}
%\label{tab:mcslam_compare}
%\vspace{-2mm}
